Uniformly polynomial-time classification of surface homeomorphisms

We describe an algorithm which, given two essential curves on a surface $S$, computes their distance in the curve graph of $S$, up to multiplicative and additive errors. As an application, we present an algorithm to decide the Nielsen-Thurston type (periodic, reducible, or pseudo-Anosov) of a mapping class of $S$. The novelty of our algorithms lies in the fact that their running time is polynomial in the size of the input and in the complexity of $S$ -- say, its Euler characteristic. This is in contrast with previously known algorithms, which run in polynomial time in the size of the input for any fixed surface $S$.

==> annular-subsurface-projection.tex <==
\usetikzlibrary{decorations.markings,fadings,spath3,calc,math,intersections,decorations.pathreplacing,hobby}

\makeatletter
\NewDocumentCommand{\tikzsetupannulussubsurfaceprojection}{}{

\path[use as bounding box] (-3.1,1.2) rectangle (2.4,-1.2);

\path (-2,.8) coordinate (corner tl) (-2,-.8) coordinate (corner bl) (2,.8) coordinate (corner tr) (2,-.8) coordinate (corner br);
\path[spath/save=left edge] (corner tl) to[out=170,in=190,looseness=.4] (corner bl);
\path[spath/save=left edge behind] (corner tl) to[dotted,out=-10,in=10,looseness=.4] (corner bl);
\path[spath/save=right edge] (corner tr) to[out=190,in=170,looseness=.4] (corner br);
\path[spath/save=right edge behind] (corner tr) to[out=10,in=-10,looseness=.4] (corner br);
\path[spath/save=top edge] (corner tl) to[bend right=10] (corner tr);
\path[spath/save=bottom edge] (corner bl) to[bend left=10] (corner br);
\tikzset{
insert left arc/.style 2 args={insert path={
(spath cs:left edge ##1) to[out=0,in=0,looseness={2}] (spath cs:left edge ##2)
}},
insert left half arc/.style={insert path={
    \ifdimcomp{##1 pt}{>}{.5pt}{
        (0,0) pic[pics/code={
            \coordinate (@tmp) at (spath cs:left edge ##1);
            \coordinate (@tmp2) at ($(0,-1.6)-(@tmp)$);
            \path[spath/save=@tmp] (@tmp) to[out=0,in=0,looseness=2.5] (@tmp2 -| @tmp);
            \path[spath/split at intersections with={@tmp}{bottom edge},spath/get components of={@tmp}{\@tmp},spath/save global=@tmp] [spath/use=\getComponentOf{\@tmp}{1}];
        }] {}
    }{
        (0,0) pic[pics/code={
            \coordinate (@tmp) at (spath cs:left edge ##1);
            \coordinate (@tmp2) at ($(0,1.6)-(@tmp)$);
            \path[spath/save=@tmp] (@tmp) to[out=0,in=0,looseness=2.5] (@tmp2 -| @tmp);
            \path[spath/split at intersections with={@tmp}{top edge},spath/get components of={@tmp}{\@tmp},spath/save global=@tmp] [spath/use=\getComponentOf{\@tmp}{1}];
        }] {} 
    } [spath/use=@tmp]
}},
insert right arc/.style 2 args={insert path={
(spath cs:right edge ##1) to[out=180,in=180,looseness={2.5}] (spath cs:right edge ##2)
}},
insert right half arc/.style={insert path={
    \ifdimcomp{##1 pt}{>}{.5pt}{
        (0,0) pic[pics/code={
            \coordinate (@tmp) at (spath cs:right edge ##1);
            \coordinate (@tmp2) at ($(0,-1.6)-(@tmp)$);
            \path[spath/save=@tmp] (@tmp) to[out=180,in=180,looseness=2.5] (@tmp2 -| @tmp);
            \path[spath/split at intersections with={@tmp}{bottom edge},spath/get components of={@tmp}{\@tmp},spath/save global=@tmp] [spath/use=\getComponentOf{\@tmp}{1}];
        }] {}
    }{
        (0,0) pic[pics/code={
            \coordinate (@tmp) at (spath cs:right edge ##1);
            \coordinate (@tmp2) at ($(0,1.6)-(@tmp)$);
            \path[spath/save=@tmp] (@tmp) to[out=180,in=180,looseness=2] (@tmp2 -| @tmp);
            \path[spath/split at intersections with={@tmp}{top edge},spath/get components of={@tmp}{\@tmp},spath/save global=@tmp] [spath/use=\getComponentOf{\@tmp}{1}];
        }] {} 
    } [spath/use=@tmp]
}},
}

\NewDocumentCommand{\otherliftsofc}{}{
\draw[palette 2,line] [insert left arc={.2}{.6},insert left arc={.72}{.9},insert left arc={.26}{.37},insert left arc={.4}{.54},insert right arc={.82}{.9},insert right half arc={.3},insert right arc={.43}{.66},insert right arc={.7}{.78}];
}
% 
\NewDocumentCommand{\annuluscontour}{}{\draw[black,line] [spath/use/.list={left edge,right edge,right edge behind,top edge,bottom edge}];}
\NewDocumentCommand{\annuluscontourbehind}{}{\draw[black,line,dotted,opacity=.3] [spath/use=left edge behind];}
\path[spath/save=@tmp 1,insert left half arc={.18}];
\tikzset{spath/remove empty components={@tmp 1}}
\path[spath/save=@tmp 1,spath/use={@tmp 1,reverse}];
\path[spath/save=@tmp 2,insert left arc={.23}{.56}];
\path[spath/save=@tmp 3,insert left arc={.62}{.68}];
\path[spath/save=@tmp 4,insert left half arc={.7}];
\tikzset{spath/remove empty components={@tmp 4}}
\path[spath/save=@tmp 5] (corner br);
\path[spath/save=@tmp 6,insert right arc={.8}{.4}];
\path[spath/save=@tmp 7,insert right arc={.38}{.32}];
\path[spath/save=@tmp 8,insert right arc={.24}{.07}];
\path[spath/save=@tmp 9] (corner tr);
\path[spath/save=Z bar boundary] \foreach \i in {1,2,3,4,6,7,8} {[spath/use=@tmp \i]};
\path[spath/save=Z bar background] [spath/use=@tmp 1] \foreach \i in {2,...,9} {to[bend right=30] (spath cs:{@tmp \i} 0) [spath/append=@tmp \i]};

\NewDocumentCommand{\clipinannulus}{m}{\begin{scope}\clip [spath/use=left edge,spath/append=bottom edge,spath/append reverse=right edge,spath/append reverse=top edge];##1\end{scope}}

\NewDocumentCommand{\Zbarcontour}{}{
    \draw[\colourmakedark{4},line] [spath/use=Z bar boundary];
}
\NewDocumentCommand{\Zbarbackground}{}{
    \clipinannulus{\fill[\colourmakebackground{4}] [spath/use=Z bar background];}
}
\path[spath/save=c bar] (spath cs:top edge .5) to[out=180,in=180,looseness=.4] (spath cs:bottom edge .5);
\NewDocumentCommand{\cbar}{}{
    \draw[palette 2,line] [spath/use=c bar];
}
\NewDocumentCommand{\cbarbehind}{}{
    \draw[palette 2,line,dotted,opacity=.3] (spath cs:top edge .5) to[out=0,in=0,looseness=.4] (spath cs:bottom edge .5);
}

\path[spath/save=Y bar contour left] (spath cs:top edge .4) to[out=180,in=180,looseness=.4] (spath cs:bottom edge .4);
\path[spath/save=Y bar contour right] (spath cs:top edge .6) to[out=180,in=180,looseness=.4] (spath cs:bottom edge .6);
\NewDocumentCommand{\Ybarbackground}{}{
    \clipinannulus{\fill[\colourmakebackground{3}] [spath/use=Y bar contour left] -- (spath cs:Y bar contour right 1) [spath/use={Y bar contour right,reverse}] -- (spath cs:Y bar contour left 0);}
}
\NewDocumentCommand{\Ybarcontour}{}{
    \draw[\colourmakedark{3},line] [spath/use=Y bar contour left,spath/use=Y bar contour right];
}

\path[spath/save=W left arc] (spath cs:left edge .69) to[out=5,in=180] (spath cs:Y bar contour left .5);
\path[spath/save=W right arc] (spath cs:Y bar contour right .5) to[out=0,in=175] (spath cs:right edge .39);
\NewDocumentCommand{\W}{}{
    \draw[palette 1,line] [spath/use/.list={W left arc,W right arc,Y bar contour left,Y bar contour right}];
}
\NewDocumentCommand{\Wbehind}{}{
    \draw[palette 1,line,dotted,opacity=.3] (spath cs:Y bar contour left 0) to[out=0,in=0,looseness=.4] (spath cs:Y bar contour left 1) (spath cs:Y bar contour right 0) to[out=0,in=0,looseness=.4] (spath cs:Y bar contour right 1);
}

\coordinate (@a) at (spath cs:W left arc .45);
\coordinate (@b) at (spath cs:bottom edge .2);
\coordinate (@c) at (spath cs:top edge .3);
\coordinate (@d) at (spath cs:Y bar contour left .4);
\coordinate (@e) at (spath cs:Y bar contour right .6);
\path[spath/save=a bar] (spath cs:left edge .4) to[out=0,in=120,in looseness=.5] (@a) to[out=-60,in=180,out looseness=.5] (@b) (@c) to[out=0,in=135,out looseness=.4] (@d) to[out=-45,in=160] (@e) to[out=-20,in=180] (spath cs:right edge .6);
\path[spath/save=a bar behind] (@b) to[out=0,in=180,looseness=.4] (@c);
\NewDocumentCommand{\abar}{}{
    \draw[line,palette 2] [spath/use=a bar];
}
\NewDocumentCommand{\abarbehind}{}{
    \draw[line,palette 2,dotted,opacity=.3] [spath/use=a bar behind];
}
\coordinate (@f) at (spath cs:bottom edge .23);
\coordinate (@g) at (spath cs:top edge .34);
\coordinate (@h) at (spath cs:bottom edge .43);
\coordinate (@i) at (spath cs:top edge .45);
\coordinate (@j) at (spath cs:bottom edge .5);
\coordinate (@k) at (spath cs:top edge .52);
\path[spath/save=f a bar] (spath cs:left edge .32) to[out=0,in=120] (@a) to[out=-60,in=180] (@f) (@g) to[out=0,in=100,looseness=.4] (@d) to[out=-80,in=180,looseness=.4] (@h) (@i) to[out=0,in=180,looseness=.4] (@j) (@k) to[out=0,in=160,out looseness=.4,in looseness=1] (@e) to[out=-20,in=180,out looseness=.5] (spath cs:right edge .5);
\path[spath/save=f a bar behind] (@f) to[out=0,in=180,looseness=.4] (@g) (@h) to[out=0,in=180,looseness=.4] (@i) (@j) to[out=0,in=180,looseness=.4] (@k);
\NewDocumentCommand{\fabar}{}{
    \draw[line,palette 3] [spath/use=f a bar];
}
\NewDocumentCommand{\fabarbehind}{}{
    \draw[line,palette 3,dotted,opacity=.3] [spath/use=f a bar behind];
}
\tikzset{wiggly/.style={
    decorate,decoration={show path construction,curveto code={
         \path[decorate,decoration={markings,mark=between positions .25 and .99 step .25 with {\coordinate (@tmp\pgfkeysvalueof{/pgf/decoration/mark info/sequence number}) at (90:rand*.1);}}] (\tikzinputsegmentfirst) .. controls(\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb) .. (\tikzinputsegmentlast);
         \tikzmath{coordinate \p,\q;\p=(\tikzinputsegmentsupporta)-(\tikzinputsegmentfirst);\q=(\tikzinputsegmentsupportb)-(\tikzinputsegmentlast);\a=atan2(\py,\px);\b=atan2(\qy,\qx);\p=(\tikzinputsegmentfirst);}
         \draw[##1] (\tikzinputsegmentfirst) to[out angle=\a,in angle=\b,curve through={(@tmp1) .. (@tmp2) .. (@tmp3)}] (\tikzinputsegmentlast);
         \ifdimcomp{\px}{<}{-2cm}{
            \coordinate (f a bar wiggly pin) at (@tmp1);
         }{}
    }}
}}
\NewDocumentCommand{\fabarwiggly}{}{
\path[wiggly={line,palette 3}] [spath/use=f a bar];
}
\NewDocumentCommand{\fabarwigglybehind}{}{
\path[wiggly={line,palette 3,dotted,opacity=.3}] [spath/use=f a bar behind];
}
\NewDocumentCommand{\intersectionsofabarandfabar}{}{
\tikzset{name intersections={of=a bar and f a bar}}
\fill[black] (intersection-4) circle (.75pt);
}

\pgfmathsetseed{6}

}
\makeatother

==> one-vertex-triangulations.tex <==
\usetikzlibrary{calc,math,spath3}

\pgfkeys{
@apply style/.style={#1},
@expand style/.style={/@apply style/.expanded={#1}},
}

\makeatletter
\tikzset{
ovt/.is family,
ovt/.cd,
new/.code={
    \edef\ovt@debug{0}
    \pgfqkeys{/tikz/ovt/@parse new}{@defaults,#1}
    \begin{scope}[shift={(\ovt@centre)}]
    \coordinate (ovt-centre) at (0,0);
    \foreach \i[evaluate=\i as \a using {360/\ovt@n*(\i+0.5)}] in {0,...,\ovt@n} {
        \coordinate (ovt-corner-\i) at (\a:\ovt@radius);
        \path[spath/save global=ovt-radial-edge-\i] (0,0) -- (ovt-corner-\i);
        \expandafter\xdef\csname ovt@inner arcs@\i\endcsname{0}
    }
    \foreach \i in {1,...,\ovt@n} {
        \path[spath/save global=ovt-outer-edge-\i] (ovt-corner-\the\numexpr\i-1\relax) -- (ovt-corner-\i);
        \expandafter\xdef\csname ovt@outer arcs@\i\endcsname{0}
        \foreach \j in {1,2,3} {
            \expandafter\xdef\csname ovt@arcs@\i @\j\endcsname{0}
        }
    }
    \foreach \cnt[count=\i,expand list] in {\ovt@arcs} {
        \pgfmathtruncatemacro\t{(\i+2)/3}
        \pgfmathtruncatemacro\c{mod(\i-1,3)+1}
        \expandafter\xdef\csname ovt@arcs@\t @\c\endcsname{\cnt}
        % \typeout{set ovt@arcs@\t @\c=\cnt}
    }
    \xdef\ovt@arcs@cnt{0}
    \xdef\ovt@traintrack{}
    \foreach \i[evaluate=\i as \j using int(\i-1)] in {1,...,\ovt@n} {
        \edef\cnta{\csname ovt@arcs@\i @1\endcsname}
        \edef\cntb{\csname ovt@arcs@\i @2\endcsname}
        \edef\cntc{\csname ovt@arcs@\i @3\endcsname}
        \edef\cntd{\the\numexpr\cntb+\cntc\relax}
        \edef\cnte{\the\numexpr\cnta+\cntc\relax}
        \edef\cntf{\the\numexpr\cnta+\cntb\relax}
        \typeout{cnta \cnta\space cntb \cntb\space cntc \cntc\space cntd \cntd\space cnte \cnte\space cntf \cntf}
        \ifnumcomp{\cnta}{>}{0}{
            \pgfmathsetmacro\outa{(\j+.5)*360/\ovt@n+90}
            \pgfmathsetmacro\ina{(\i+.5)*360/\ovt@n-90}
            \xdef\ovt@traintrack{\ovt@traintrack,insert path={($(ovt-centre)!.5!(ovt-corner-\j)$) to[out=\outa,in=\ina] ($(ovt-centre)!.5!(ovt-corner-\i)$)}}
            \foreach \k in {1,...,\cnta} {
                \pgfmathsetmacro\p{\k/(\cntf+1)*.5+.25}
                \pgfmathsetmacro\q{\k/(\cnte+1)*.5+.25}
                \xdef\ovt@arcs@cnt{\the\numexpr\ovt@arcs@cnt+1\relax}
                \path[spath/save global=ovt-arc-\ovt@arcs@cnt] ($(ovt-centre)!\p!(ovt-corner-\j)$) to[out=\outa,in=\ina] ($(ovt-centre)!\q!(ovt-corner-\i)$);
            }
        }{}
        \ifnumcomp{\cntb}{>}{0}{
            \pgfmathsetmacro\outa{(\j+.5)*360/\ovt@n+90}
            \pgfmathsetmacro\ina{\i*360/\ovt@n-180}
            \xdef\ovt@traintrack{\ovt@traintrack,insert path={($(ovt-corner-\j)!.5!(ovt-centre)$) to[out=\outa,in=\ina] ($(ovt-corner-\j)!.5!(ovt-corner-\i)$)}}
            \foreach \k in {1,...,\cntb} {
                \pgfmathsetmacro\p{\k/(\cntf+1)*.5+.25}
                \pgfmathsetmacro\q{\k/(\cntd+1)*.5+.25}
                \xdef\ovt@arcs@cnt{\the\numexpr\ovt@arcs@cnt+1\relax}
                \path[spath/save global=ovt-arc-\ovt@arcs@cnt] ($(ovt-corner-\j)!\p!(ovt-centre)$) to[out=\outa,in=\ina,looseness=.8] ($(ovt-corner-\j)!\q!(ovt-corner-\i)$);
            }
        }{}
        \ifnumcomp{\cntc}{>}{0}{
            \pgfmathsetmacro\outa{(\i+.5)*360/\ovt@n-90}
            \pgfmathsetmacro\ina{\i*360/\ovt@n-180}
            \xdef\ovt@traintrack{\ovt@traintrack,insert path={($(ovt-corner-\i)!.5!(ovt-centre)$) to[out=\outa,in=\ina,looseness=.8] ($(ovt-corner-\i)!.5!(ovt-corner-\j)$)}}
            \foreach \k in {1,...,\cntc} {
                \pgfmathsetmacro\p{\k/(\cnte+1)*.5+.25}
                \pgfmathsetmacro\q{\k/(\cntd+1)*.5+.25}
                \xdef\ovt@arcs@cnt{\the\numexpr\ovt@arcs@cnt+1\relax}
                \path[spath/save global=ovt-arc-\ovt@arcs@cnt] ($(ovt-corner-\i)!\p!(ovt-centre)$) to[out=\outa,in=\ina,looseness=.8] ($(ovt-corner-\i)!\q!(ovt-corner-\j)$);
            }
        }{}
    }
    \ifnumcomp{\ovt@debug}{=}{1}{
        \foreach \i[evaluate=\i as \j using int(\i-1)] in {1,...,\ovt@n} {
            \draw[line] (ovt-centre) -- (ovt-corner-\i) node[midway,scale=.5] {\contour{white}{\i}};
            \draw[line] (ovt-corner-\j) -- (ovt-corner-\i) node[midway,scale=.5] {\contour{white}{\i}};
        }
        % \draw[blue,line] [/@expand style={\ovt@traintrack}];
        \foreach \j in {1,...,\ovt@arcs@cnt} {
            \draw[line,red] [spath/use=ovt-arc-\j];
            \node[red,scale=.3] at (spath cs:{ovt-arc-\j} .5) {\contour{white}{\j}};
        }
    }{}
    \end{scope}
},
every label in corner/.style={},
label in corner/.code n args={4}{
\pgfmathsetmacro\r{\ovt@radius/6+1pt}
\ifnumcomp{#2}{=}{1}{
\pgfmathsetmacro\a{360/\ovt@n*#1}
\pgfmathsetmacro\r{\r+3pt}
\coordinate (ovt@tmp) at (ovt-centre);
}{}
\ifnumcomp{#2}{=}{2}{
\pgfmathsetmacro\a{135+360/\ovt@n*(#1-.25)}
\coordinate (ovt@tmp) at (ovt-corner-\the\numexpr#1-1\relax);
}{}
\ifnumcomp{#2}{=}{3}{
\pgfmathsetmacro\a{-135+360/\ovt@n*(#1+.25)}
\coordinate (ovt@tmp) at (ovt-corner-#1);
}{}
\node[anchor=center,ovt/every label in corner,#3] at ($(ovt@tmp)+(\a:\r pt)$) {#4};
},
}

\tikzset{
ovt/@parse new/.is family,
ovt/@parse new/.cd,
n/.code={\xdef\ovt@n{#1}},
radius/.code={\xdef\ovt@radius{#1}},
centre/.estore in=\ovt@centre,
arcs/.estore in=\ovt@arcs,
debug/.code={\edef\ovt@debug{1}},
@defaults/.style={
centre={0,0},
radius=2cm,
arcs={}
}
}

\NewDocumentCommand{\ovt@createpathretrievalcommands}{mmmm}{
    \tikzset{
        ovt/.cd,
        #1/.code={
            \foreach #3 in {##1} {
                \tikzset{/@expand style={#4}}
            }
        },
        #1 all/.code={
            \foreach #3 in {1,...,#2} {
                \tikzset{/@expand style={#4}}
            }
        },
        #1 all but/.code={
            \foreach #3 in {1,...,#2} {
                \xdef\ovt@createpathretrievalcommands@ok{1}
                \foreach \ovt@createpathretrievalcommands@i in {##1} {
                    \ifthenelse{#3=\ovt@createpathretrievalcommands@i}{
                        \xdef\ovt@createpathretrievalcommands@ok{0}
                    }{}
                }
                \ifthenelse{\ovt@createpathretrievalcommands@ok=1}{
                    \tikzset{/@expand style={#4}}
                }{}
            }
        }
    }
}

\ovt@createpathretrievalcommands{use radial edge}{\ovt@n}{\i}{spath/use=ovt-radial-edge-\i}
\ovt@createpathretrievalcommands{use outer edge}{\ovt@n}{\i}{spath/use=ovt-outer-edge-\i}
\ovt@createpathretrievalcommands{use arc}{\ovt@arcs@cnt}{\i}{spath/use=ovt-arc-\i}
\tikzset{
ovt/use train track/.style={/@expand style={\ovt@traintrack}},
}







\makeatother

==> train-tracks.tex <==

\usetikzlibrary{arrows.meta, calc, decorations.markings, decorations.pathreplacing, intersections, math, spath3}
\ifarXiv{}{
\usetikzlibrary{nfold}
}

\makeatletter

\def\tt@MAXBRANCHES{99}

\pgfkeys{
@apply style/.style={#1},
@expand style/.style={/@apply style/.expanded={#1}},
}

% inspired by https://tex.stackexchange.com/questions/422657/check-for-group-as-argument-expandable
\def\tt@ifstartswithbrace#1{\tt@ifstartswithbrace@ #1.{}\end}
\def\tt@ifstartswithbrace@#1#{\ifx\end#1\end\expandafter\tt@ifstartswithbrace@T
   \else\expandafter\tt@ifstartswithbrace@F\fi}
\def\tt@ifstartswithbrace@T#1\end{\@firstoftwo}
\def\tt@ifstartswithbrace@F#1\end{\@secondoftwo}


\tikzset{
tt/.is family,
tt/.cd,
new/.code={
    \expandafter\xdef\csname TT@#1@switches@n\endcsname{0}
    \expandafter\xdef\csname TT@#1@branches@n\endcsname{0}
    \expandafter\xdef\csname TT@#1@width\endcsname{}
    \expandafter\xdef\csname TT@#1@sep\endcsname{}
    \expandafter\xdef\csname TT@#1@spread\endcsname{}
    \newboolean{TT@#1@isfinalised}
    \newboolean{TT@#1@isthick}
    \tt@newsequence{TT@#1@bunches@right}
    \tt@newsequence{TT@#1@bunches@left}
    \tt@newsequence{TT@#1@bunches@above}
    \tt@newsequence{TT@#1@bunches@below}
    \tt@newsequence{TT@#1@bunches@between}
    \foreach \i in {1,...,\tt@MAXBRANCHES} {
        \expandafter\xdef\csname TT@#1@branch@\i @weight\endcsname{0}
    }
    \tikzset{
        tt/#1/.is family,
        tt/#1/.cd,
        .unknown/.code={
            \def\tt@unknown@value{##1}
            \let\tt@unknown@key=\pgfkeyscurrentname
            % \typeout{\tt@unknown@key : \tt@unknown@value}
            \tt@ifstartswithbrace{##1}{
                \pgfqkeys{/tikz/tt}{
                    \tt@unknown@key={#1}##1
                }
            }{
                \ifthenelse{\pdfstrcmp{##1}{}=0}{
                    \pgfqkeys{/tikz/tt}{
                        \tt@unknown@key={#1}
                    }
                }{
                    \pgfqkeys{/tikz/tt}{
                        \tt@unknown@key={#1}{##1}
                    }
                }
            }
            
        }
    }
},
set spread/.code 2 args={
    \tt@ensurenotfinalised{#1}
    \expandafter\xdef\csname TT@#1@spread\endcsname{#2}
},
set sep/.code 2 args={
    \tt@ensurenotfinalised{#1}
    \expandafter\xdef\csname TT@#1@sep\endcsname{#2}
},
set width/.code 2 args={
    \tt@ensurenotfinalised{#1}
    \expandafter\xdef\csname TT@#1@width\endcsname{#2}
},
add switch/.code 2 args={
    \tt@ensurenotfinalised{#1}
    \edef\n{\the\numexpr\csname TT@#1@switches@n\endcsname+1}
    \expandafter\xdef\csname TT@#1@switches@n\endcsname{\n}
    \expandafter\xdef\csname TT@#1@switch@\n @thickness\endcsname{0}
    \tikzset{
        tt/set switch spread={#1}{\n}{\csname TT@#1@spread\endcsname},
        tt/set switch sep={#1}{\n}{\csname TT@#1@sep\endcsname},
        tt/set switch width={#1}{\n}{\csname TT@#1@width\endcsname},
    }
    \tt@newproplist{TT@#1@switch@\n @bunches}
    \coordinate (\ttswitch{#1}{\n}) at (#2);
    \coordinate (#1-\n) at (#2);
},
set switch thickness/.code n args={3}{
    \tt@ensurenotfinalised{#1}
    \ifthenelse{\boolean{TT@#1@isthick}}{
        \PackageWarning{tt}{Overwriting previously set thickness for switch \csname TT@#1@thickness@switch\endcsname}
    }{}
    \setboolean{TT@#1@isthick}{true}
    \expandafter\xdef\csname TT@#1@thickness@switch\endcsname{#2}
    \expandafter\xdef\csname TT@#1@thickness\endcsname{#3}
},
set switch width/.code n args={3}{
    \tt@ensurenotfinalised{#1}
    \expandafter\xdef\csname TT@#1@switch@#2@width\endcsname{#3}
},
set switch spread/.code n args={3}{
    \tt@ensurenotfinalised{#1}
    \expandafter\xdef\csname TT@#1@switch@#2@spread\endcsname{#3}
    \expandafter\xdef\csname TT@#1@switch@#2@spread@l\endcsname{#3}
    \expandafter\xdef\csname TT@#1@switch@#2@spread@r\endcsname{#3}
},
set switch spread left/.code n args={3}{
    \tt@ensurenotfinalised{#1}
    \expandafter\xdef\csname TT@#1@switch@#2@spread@l\endcsname{#3}
},
set switch spread right/.code n args={3}{
    \tt@ensurenotfinalised{#1}
    \expandafter\xdef\csname TT@#1@switch@#2@spread@r\endcsname{#3}
},
set switch sep/.code n args={3}{
    \tt@ensurenotfinalised{#1}
    \expandafter\xdef\csname TT@#1@switch@#2@sep\endcsname{#3}
    \expandafter\xdef\csname TT@#1@switch@#2@sep@l\endcsname{#3}
    \expandafter\xdef\csname TT@#1@switch@#2@sep@r\endcsname{#3}
},
set switch sep left/.code n args={3}{
    \tt@ensurenotfinalised{#1}
    \expandafter\xdef\csname TT@#1@switch@#2@sep@l\endcsname{#3}
},
set switch sep right/.code n args={3}{
    \tt@ensurenotfinalised{#1}
    \expandafter\xdef\csname TT@#1@switch@#2@sep@r\endcsname{#3}
},
add branch/.code 2 args={
    \tt@ensurenotfinalised{#1}
    \edef\n{\the\numexpr\csname TT@#1@branches@n\endcsname+1}
    \expandafter\xdef\csname TT@#1@branches@n\endcsname{\n}
    \expandafter\xdef\csname TT@#1@branch@\n @weight\endcsname{0}
    \expandafter\xdef\csname TT@#1@branch@\n @frombunch\endcsname{0}
    \path[spath/save global=\ttbranch{#1}{\n}] #2;
    \tikzset{tt/@find closest switch={#1}{spath cs:{\ttbranch{#1}{\n}} 0}{.01pt}}
    \expandafter\xdef\csname TT@#1@branch@\n @begin\endcsname{\tt@result}
    \tikzset{tt/@find closest switch={#1}{spath cs:{\ttbranch{#1}{\n}} 1}{.01pt}}
    \expandafter\xdef\csname TT@#1@branch@\n @end\endcsname{\tt@result}
},
add branch standard/.style n args={3}{
    add branch={#1}{(\ttswitch{#1}{#2}) to[out=0,in=180] (\ttswitch{#1}{#3})}
},
set branch weight/.code n args={3}{
    \tt@ensurenotfinalised{#1}
    % \setboolean{TT@#1@isthick}{true}
    \pgfmathparse{int(#3)}
    \expandafter\xdef\csname TT@#1@branch@#2@weight\endcsname{\pgfmathresult}
},
set branch weights/.code 2 args={
    \edef\tt@setbranchweights@currenttt{#1}
    \pgfqkeys{/tikz/tt/@set branch weights}{#2}
},
@set branch weights/.is family,
@set branch weights/.unknown/.style={/tikz/tt/set branch weight={\tt@setbranchweights@currenttt}{\pgfkeyscurrentname}{#1}},
add bunch/.code n args={4}{
    \tt@ensurenotfinalised{#1}
    \tt@addtoproplist{TT@#1@switch@#2@bunches}{#3}{#4}
},
finalise/.code={
    \tt@ensurenotfinalised{#1}
    \ifnumcomp{\csname TT@#1@switches@n\endcsname}{>}{0}{
        \foreach \i in {1,...,\csname TT@#1@switches@n\endcsname} {
            \tt@newsequence{TT@#1@switch@\i @adj@l}
            \tt@newsequence{TT@#1@switch@\i @adj@r}
        }
    }{}
    \ifnumcomp{\csname TT@#1@branches@n\endcsname}{>}{0}{
        \foreach \i in {1,...,\csname TT@#1@branches@n\endcsname} {
            \foreach \j/\end in {\csname TT@#1@branch@\i @begin\endcsname/begin,\csname TT@#1@branch@\i @end\endcsname/end} {
                \ifthenelse{\j=0}{}{
                    \tikzset{tt/point along branch={#1}{\i}{\end,8pt,name=tt@tmp}}
                    \path let \p1=($(tt@tmp)-(\ttswitch{#1}{\j})$) in \pgfextra{
                        \ifdimcomp{\x1}{<}{0pt}{
                            \tt@addtosequence{TT@#1@switch@\j @adj@l}{\y1,\i,\end}
                        }{
                            \tt@addtosequence{TT@#1@switch@\j @adj@r}{\y1,\i,\end}
                        }
                    };
                }
            }
        }
    }{}
    \ifnumcomp{\csname TT@#1@switches@n\endcsname}{>}{0}{
        \foreach \i in {1,...,\csname TT@#1@switches@n\endcsname} {
            \tt@sortadjacencylist{TT@#1@switch@\i @adj@l}{TT@#1@switch@\i @adj@l@ends}
            \tt@sortadjacencylist{TT@#1@switch@\i @adj@r}{TT@#1@switch@\i @adj@r@ends}
        }
    }{}
    % % add bunched branches
    \xdef\tt@finalise@donesomething{0}
    \ifnumcomp{\csname TT@#1@switches@n\endcsname}{>}{0}{
        \foreach \i in {1,...,\csname TT@#1@switches@n\endcsname} {
            \ifthenelse{\tt@proplistlength{TT@#1@switch@\i @bunches}>0}{
                \xdef\tt@finalise@donesomething{1}
            }{}
            \foreach \dir/\dirfullname in {l/left,r/right} {
                \edef\n{\tt@sequencelength{TT@#1@switch@\i @adj@\dir}}
                \ifthenelse{\n=0}{
                    % process bunch of the form "left"/"right"
                    \csname tt@processbunch\dirfullname\endcsname{#1}{\i}
                }{
                    \edef\br{\tt@getfromsequence{TT@#1@switch@\i @adj@\dir}{1}}
                    \edef\end{\tt@getfromsequence{TT@#1@switch@\i @adj@\dir @ends}{1}}
                    % process bunch of the form "above \br"
                    \tt@processbunchabove{#1}{\i}{\dir}{\br}{\end}
                    % process bunches of the form "between ..."
                    \ifthenelse{\n>1}{
                        \foreach \j[evaluate=\j as \jj using {int(\j-1)}] in {2,...,\n} {
                            \edef\br{\tt@getfromsequence{TT@#1@switch@\i @adj@\dir}{\j}}
                            \edef\end{\tt@getfromsequence{TT@#1@switch@\i @adj@\dir @ends}{\j}}
                            \edef\brr{\tt@getfromsequence{TT@#1@switch@\i @adj@\dir}{\jj}}
                            \edef\endd{\tt@getfromsequence{TT@#1@switch@\i @adj@\dir @ends}{\jj}}
                            \tt@processbunchbetween{#1}{\i}{\dir}{\brr}{\endd}{\br}{\end}
                        }
                    }{}
                    \edef\br{\tt@getfromsequence{TT@#1@switch@\i @adj@\dir}{\n}}
                    \edef\end{\tt@getfromsequence{TT@#1@switch@\i @adj@\dir @ends}{\n}}
                    % process bunch of the form "below \br"
                    \tt@processbunchbelow{#1}{\i}{\dir}{\br}{\end}
                }
            }
            \tt@warnforinvalidbunches{\i}{TT@#1@switch@\i @bunches}
            \tt@newproplist{TT@#1@switch@\i @bunches}
        }
    }{}
    \ifthenelse{\tt@finalise@donesomething=1}{
        \tikzset{tt/finalise={#1}}
    }{
        \ifthenelse{\boolean{TT@#1@isthick}}{
            %compute branch thicknesses
            \edef\sw{\csname TT@#1@thickness@switch\endcsname}
            \def\dir{r}
            \ifthenelse{\tt@sequencelength{TT@#1@switch@\sw @adj@l}>0}{
                \def\dir{l}
            }{}
            \xdef\tt@totalweight{0}
            \foreach \i in {1,...,\tt@sequencelength{TT@#1@switch@\sw @adj@\dir}}{
                \edef\j{\tt@getfromsequence{TT@#1@switch@\sw @adj@\dir}{\i}}
                \edef\w{\csname TT@#1@branch@\j @weight\endcsname}
                \xdef\tt@totalweight{\the\numexpr\tt@totalweight+\w}
            }
            \ifthenelse{\tt@totalweight=0}{
                \PackageWarning{tt}{Switch \sw\space only has branches of weight 0 on one side} 
            }{
                \pgfmathparse{(\csname TT@#1@thickness\endcsname)/\tt@totalweight}
                \edef\tt@unitthickness{\pgfmathresult}
                \foreach \i in {1,...,\csname TT@#1@branches@n\endcsname}{
                    \edef\w{\csname TT@#1@branch@\i @weight\endcsname}
                    \pgfmathparse{\w*\tt@unitthickness}
                    \expandafter\xdef\csname TT@#1@branch@\i @thickness\endcsname{\pgfmathresult pt}
                    % \typeout{Branch \i\space has thickness \pgfmathresult pt}
                }
                % compute switch thicknesses
                \foreach \i in {1,...,\csname TT@#1@branches@n\endcsname}{
                    \path[spath/use=\ttbranch{#1}{\i}] coordinate[pos=0] (tt@branch@\i @newbegin) coordinate[pos=1] (tt@branch@\i @newend);
                }
                \foreach \i in {1,...,\csname TT@#1@switches@n\endcsname}{
                    \foreach \dir in {l,r} {
                        \expandafter\def\csname tt@thickness@\dir\endcsname{0}
                        \foreach \j in {1,...,\tt@sequencelength{TT@#1@switch@\i @adj@\dir}}{
                            \edef\k{\tt@getfromsequence{TT@#1@switch@\i @adj@\dir}{\j}}
                            \edef\w{\csname TT@#1@branch@\k @weight\endcsname}
                            \expandafter\pgfmathparse{int(\w+\csname tt@thickness@\dir\endcsname)}
                            \expandafter\xdef\csname tt@thickness@\dir\endcsname{\pgfmathresult}
                        }
                    }
                    % \typeout{Switch \i\space has thickness \tt@thickness@l\space on the left and \tt@thickness@r\space on the right}
                    \pgfmathparse{int(abs(\tt@thickness@l-\tt@thickness@r))}
                    \ifthenelse{\pgfmathresult=0}{}{
                        \PackageWarning{tt}{Switch \i\space has weight \tt@thickness@l\space on the left and weight \tt@thickness@r\space on the right}
                    }
                    \pgfmathparse{\tt@thickness@l*\tt@unitthickness}
                    \edef\tt@thickness@l{\pgfmathresult}
                    \pgfmathparse{\tt@thickness@r*\tt@unitthickness}
                    \edef\tt@thickness@r{\pgfmathresult}
                    \pgfmathparse{max(\tt@thickness@l,\tt@thickness@r)}
                    \edef\tt@thickness{\pgfmathresult}
                    \expandafter\xdef\csname TT@#1@switch@\i @thickness\endcsname{\tt@thickness pt}
                    % compute new endpoints of incident branches
                    \foreach \dir/\dirmult in {l/-1,r/1} {
                        \pgfmathparse{(\csname TT@#1@switch@\i @width\endcsname)/2*(\dirmult)}
                        \edef\dx{\pgfmathresult}
                        \pgfmathparse{(\csname tt@thickness@\dir\endcsname)/2}
                        \xdef\tt@dy{\pgfmathresult}
                        \foreach \j in {1,...,\tt@sequencelength{TT@#1@switch@\i @adj@\dir}} {
                            \edef\k{\tt@getfromsequence{TT@#1@switch@\i @adj@\dir}{\j}}
                            \edef\end{\tt@getfromsequence{TT@#1@switch@\i @adj@\dir @ends}{\j}}
                            \edef\t{\csname TT@#1@branch@\k @thickness\endcsname}
                            \pgfmathparse{\tt@dy-\t/2}
                            \edef\tt@dy{\pgfmathresult}
                            \coordinate (tt@branch@\k @new\end) at ([shift={(\dx pt,\tt@dy pt)}]\ttswitch{#1}{\i});
                            \pgfmathparse{\tt@dy-\t/2}
                            \xdef\tt@dy{\pgfmathresult}
                        }
                    }
                }
                % adjust endpoints of branches
                \foreach \i in {1,...,\csname TT@#1@branches@n\endcsname}{
                    \ifthenelse{\csname TT@#1@branch@\i @frombunch\endcsname=0} {
                        \tt@adjustendpointsofbranch{\ttbranch{#1}{\i}}{tt@branch@\i @newbegin}{tt@branch@\i @newend}
                    }
                }
                % reprocess bunches
                \foreach \kind in {left,right,above,below,between} {
                    \ifthenelse{\tt@sequencelength{TT@#1@bunches@\kind}>0}{
                        \foreach \i in {1,...,\tt@sequencelength{TT@#1@bunches@\kind}} {
                            \edef\j{\tt@getfromsequence{TT@#1@bunches@\kind}{\i}}
                            \csname tt@thick@processbunch\kind\endcsname{#1}{\j}
                        }
                    }{}
                }
                % save paths for future use
                \foreach \i in {1,...,\csname TT@#1@switches@n\endcsname} {
                    \edef\w{\csname TT@#1@switch@\i @width\endcsname}
                    \edef\h{\csname TT@#1@switch@\i @thickness\endcsname}
                    \begin{scope}[shift=(\ttswitch{#1}{\i})]
                        \path[spath/save global=tt@#1@switch@\i @upper contour] (-\w/2,\h/2) -- (\w/2,\h/2);
                        \path[spath/save global=tt@#1@switch@\i @lower contour] (-\w/2,-\h/2) -- (\w/2,-\h/2);
                        \path[spath/save global=tt@#1@switch@\i @contour] [spath/use=tt@#1@switch@\i @upper contour,spath/use=tt@#1@switch@\i @lower contour];
                        \path[spath/save global=tt@#1@switch@\i @background] ({-\w/2-0.01pt},-\h/2) rectangle ({\w/2+0.01pt},\h/2);
                    \end{scope}
                }
                \foreach \i in {1,...,\csname TT@#1@branches@n\endcsname} {
                    \tikzset{
                        spath/offset={\ttbranch{#1}{\i}}{\csname TT@#1@branch@\i @thickness\endcsname/2}{tt@#1@branch@\i @left contour},
                        spath/offset={\ttbranch{#1}{\i}}{-\csname TT@#1@branch@\i @thickness\endcsname/2}{tt@#1@branch@\i @right contour},
                    }
                    \path[spath/save global=tt@#1@branch@\i @contour] [spath/use=tt@#1@branch@\i @left contour,spath/use=tt@#1@branch@\i @right contour];
                    \path[spath/save global=tt@#1@branch@\i @background] [spath/use=tt@#1@branch@\i @left contour] -- (spath cs: {tt@#1@branch@\i @right contour} 1) [spath/use={tt@#1@branch@\i @right contour,reverse,weld}] -- cycle;
                }
            }
        }{}
        \setboolean{TT@#1@isfinalised}{true}
    }
},
debug/.code={
    \ifnumcomp{\csname TT@#1@branches@n\endcsname}{>}{0}{
        \foreach \i in {1,...,\csname TT@#1@branches@n\endcsname} {
            \edef\w{\csname TT@#1@branch@\i @weight\endcsname}
            \path[/pgf/fpu/install only={reciprocal},decorate,decoration={markings,mark=at position .5 with {\coordinate (tt@tmp);}}] [spath/use=\ttbranch{#1}{\i}];
            \ifthenelse{\w>0} {
                \edef\thickness{\csname TT@#1@branch@\i @thickness\endcsname}
                % \typeout{thickness of branch \i\space is \thickness}
                \fill[shift=(tt@tmp),gray!30] (2pt,{.5*\thickness}) rectangle (-2pt,{-.5*\thickness});
            }{}
            \draw[/pgf/fpu/install only={reciprocal},postaction={decorate,decoration={markings,mark=at position 0.45 with {\arrow{Stealth[scale=.5]}}}}] [spath/use=\ttbranch{#1}{\i}];
            \node[name=tt@tmp,scale=.5,inner sep=0pt] at (tt@tmp) {\textbf{\tikzcontour{\i}}};
            \ifthenelse{\w>0}{
                \node[scale=.3,gray,anchor=west,inner sep=0pt] at ([xshift=1pt]tt@tmp.south east) {\textbf{\tikzcontour{\w}}};
            }{}
        }
    }{}
    \ifnumcomp{\csname TT@#1@switches@n\endcsname}{>}{0}{
        \foreach \i in {1,...,\csname TT@#1@switches@n\endcsname}{
            \begin{scope}[shift={(\ttswitch{#1}{\i})}]
            \node[red!50!black,circle,draw,fill=white,inner sep=.2pt]{\textbf{\i}};
            \end{scope}
        }
    }{}
},
carried/.code 2 args={
    \tt@ensurefinalised{#1}
    \edef\tt@carried@carrying@name{#1}
    \edef\tt@carried@segments@n{0}
    \tikzset{tt/@parse carried/.cd,defaults,#2}
    \foreach \b in {1,...,\csname TT@#1@branches@n\endcsname} {
        \edef\n{\csname tt@carried@carrying@branch@\b @n\endcsname}
        \ifnumcomp{\n}{>}{0}{
            \expandafter\xdef\csname tt@carried@carrying@branch@\b @segments@begin\endcsname{\the\numexpr\tt@carried@segments@n+1}
            \edef\thickness{\csname TT@#1@branch@\b @thickness\endcsname}
            \edef\sep{\the\numexpr\thickness/\n}
            \foreach \i in {1,...,\n} {
                \xdef\tt@carried@segments@n{\the\numexpr\tt@carried@segments@n+1}
                \tikzset{spath/offset={\ttbranch{#1}{\b}}{-\thickness/2+(\i-0.5)*\sep}{tt@carried@segment@\tt@carried@segments@n}}
                \expandafter\xdef\csname tt@carried@segment@\tt@carried@segments@n @visited\endcsname{0}
                \expandafter\xdef\csname tt@carried@segment@\tt@carried@segments@n @begin@switch\endcsname{0}
                \expandafter\xdef\csname tt@carried@segment@\tt@carried@segments@n @end@switch\endcsname{0}
                % \draw[red] [spath/use=tt@carried@segment@\tt@carried@segments@n];
            }
            \expandafter\xdef\csname tt@carried@carrying@branch@\b @segments@end\endcsname{\tt@carried@segments@n}
        }{}
    }
    \foreach \s in {1,...,\csname TT@#1@switches@n\endcsname} {
        \foreach \dir in {l,r} {
            \expandafter\xdef\csname tt@carried@carrying@switch@\s @adj@\dir @n\endcsname{0}
            \foreach \k in {1,...,\tt@sequencelength{TT@#1@switch@\s @adj@\dir}} {
                \edef\b{\tt@getfromsequence{TT@#1@switch@\s @adj@\dir}{\k}}
                \edef\end{\tt@getfromsequence{TT@#1@switch@\s @adj@\dir @ends}{\k}}
                % \edef\nsegments{\csname tt@carried@carrying@branch@\b @n\endcsname}
                \ifnumcomp{\csname tt@carried@carrying@branch@\b @n\endcsname}{>}{0}{
                    \ifboolexpr{
                        (test {\ifnumcomp{\pdfstrcmp{\end}{begin}}{=}{0}} and test {\ifnumcomp{\pdfstrcmp{\dir}{l}}{=}{0}})
                        or
                        (test {\ifnumcomp{\pdfstrcmp{\end}{end}}{=}{0}} and test {\ifnumcomp{\pdfstrcmp{\dir}{r}}{=}{0}})
                    }{
                        \def\tt@carried@myf{\the\numexpr\csname tt@carried@carrying@branch@\b @segments@begin\endcsname-1+\i\relax}
                    }{
                        \def\tt@carried@myf{\the\numexpr\csname tt@carried@carrying@branch@\b @segments@end\endcsname+1-\i\relax}
                    }
                    \foreach \i in {1,...,\csname tt@carried@carrying@branch@\b @n\endcsname} {
                        \edef\j{\the\numexpr\csname tt@carried@carrying@switch@\s @adj@\dir @n\endcsname+1}
                        \expandafter\xdef\csname tt@carried@carrying@switch@\s @adj@\dir @n\endcsname{\j}
                    %     % \expandafter\xdef\csname tt@carried@carrying@switch@\s @adj@\dir @\j @branch\endcsname{\b}
                        \expandafter\xdef\csname tt@carried@carrying@switch@\s @adj@\dir @\j @end\endcsname{\end}
                        \ifnumcomp{\pdfstrcmp{\end}{begin}}{=}{0}{
                            \coordinate (tt@carried@carrying@switch@\s @adj@\dir @\j @point) at (spath cs:{tt@carried@segment@\tt@carried@myf} 0);
                        }{
                            \coordinate (tt@carried@carrying@switch@\s @adj@\dir @\j @point) at (spath cs:{tt@carried@segment@\tt@carried@myf} 1);
                        }
                        \expandafter\xdef\csname tt@carried@carrying@switch@\s @adj@\dir @\j @idx\endcsname{\tt@carried@myf}
                        \expandafter\xdef\csname tt@carried@carrying@switch@\s @adj@\dir @\j @free\endcsname{1}
                        \expandafter\xdef\csname tt@carried@carrying@switch@\s @adj@\dir @\j @mate\endcsname{0}
                        \expandafter\xdef\csname tt@carried@carrying@switch@\s @adj@\dir @\j @afterpath\endcsname{}
                        \expandafter\xdef\csname tt@carried@segment@\tt@carried@myf @\end @dir\endcsname{\dir}
                        \expandafter\xdef\csname tt@carried@segment@\tt@carried@myf @\end @idx\endcsname{\j}
                        \expandafter\xdef\csname tt@carried@segment@\tt@carried@myf @\end @switch\endcsname{\s}
                    }
                }{}
            }
        }
    }
    \ifnumcomp{\csname TT@\tt@carried@name @switches@n\endcsname}{>}{0}{
        \foreach \s in {1,...,\csname TT@\tt@carried@name @switches@n\endcsname} {
            \edef\z{\csname tt@carried@switch@\s @parentswitch\endcsname}
            \foreach \dir in {l,r} {
                \foreach \i[expand list] in {\csname tt@carried@switch@\s @adj@\dir\endcsname} {
                    \expandafter\xdef\csname tt@carried@carrying@switch@\z @adj@\dir @\i @free\endcsname{0}
                    \expandafter\xdef\csname tt@carried@carrying@switch@\z @adj@\dir @\i @afterpath\endcsname{insert path={
                            \ifnumcomp{\pdfstrcmp{\dir}{l}}{=}{0}{
                                (tt@carried@carrying@switch@\z @adj@\dir @\i @point) to[out=0,in=180] (\ttswitch{\tt@carried@name}{\s})
                            }{
                                (tt@carried@carrying@switch@\z @adj@\dir @\i @point) to[out=180,in=0] (\ttswitch{\tt@carried@name}{\s})
                            }
                        }}
                }
            }
        }
    }{}
    \foreach \z in {1,...,\csname TT@#1@switches@n\endcsname} {
        \foreach \tt@il/\tt@ir[expand list] in {\csname tt@carried@carrying@switch@\z @matches\endcsname} {
            \expandafter\xdef\csname tt@carried@carrying@switch@\z @adj@l@\tt@il @free\endcsname{0}
            \expandafter\xdef\csname tt@carried@carrying@switch@\z @adj@l@\tt@il\endcsname{0}
            \expandafter\xdef\csname tt@carried@carrying@switch@\z @adj@l@\tt@il @mate\endcsname{\tt@ir}
            \expandafter\xdef\csname tt@carried@carrying@switch@\z @adj@l@\tt@il @afterpath\endcsname{insert path={(tt@carried@carrying@switch@\z @adj@l@\tt@il @point) to[out=0,in=180] (tt@carried@carrying@switch@\z @adj@r@\tt@ir @point)}}
            \expandafter\xdef\csname tt@carried@carrying@switch@\z @adj@r@\tt@ir @free\endcsname{0}
            \expandafter\xdef\csname tt@carried@carrying@switch@\z @adj@r@\tt@ir @mate\endcsname{\tt@il}
            \expandafter\xdef\csname tt@carried@carrying@switch@\z @adj@r@\tt@ir @afterpath\endcsname{insert path={(tt@carried@carrying@switch@\z @adj@r@\tt@ir @point) to[out=180,in=0] (tt@carried@carrying@switch@\z @adj@l@\tt@il @point)}}
        }
    }
    \foreach \s in {1,...,\csname TT@#1@switches@n\endcsname} {
        \xdef\tt@li{1}
        \xdef\tt@ri{1}
        \unlessboolexpr{test {\ifnumcomp{\tt@li}{>}{\csname tt@carried@carrying@switch@\s @adj@l@n\endcsname}} or test {\ifnumcomp{\tt@ri}{>}{\csname tt@carried@carrying@switch@\s @adj@r@n\endcsname}}}{
                \ifnumcomp{\csname tt@carried@carrying@switch@\s @adj@l@\tt@li @free\endcsname}{=}{0}{
                \xdef\tt@li{\the\numexpr\tt@li+1}
            }{
                \ifnumcomp{\csname tt@carried@carrying@switch@\s @adj@r@\tt@ri @free\endcsname}{=}{0}{
                    \xdef\tt@ri{\the\numexpr\tt@ri+1}
                }{
                    % pair up \tt@li and \tt@ri
                    \expandafter\xdef\csname tt@carried@carrying@switch@\s @adj@l@\tt@li @afterpath\endcsname{insert path={(tt@carried@carrying@switch@\s @adj@l@\tt@li @point) to[out=0,in=180] (tt@carried@carrying@switch@\s @adj@r@\tt@ri @point)}}
                    \expandafter\xdef\csname tt@carried@carrying@switch@\s @adj@l@\tt@li @mate\endcsname{\tt@ri}
                    \expandafter\xdef\csname tt@carried@carrying@switch@\s @adj@r@\tt@ri @afterpath\endcsname{insert path={(tt@carried@carrying@switch@\s @adj@r@\tt@ri @point) to[out=180,in=0] (tt@carried@carrying@switch@\s @adj@l@\tt@li @point)}}
                    \expandafter\xdef\csname tt@carried@carrying@switch@\s @adj@r@\tt@ri @mate\endcsname{\tt@li}
                    \xdef\tt@li{\the\numexpr\tt@li+1}
                    \xdef\tt@ri{\the\numexpr\tt@ri+1}
                }
            }
        }
    }
    \foreach \i in {1,...,\csname tt@carried@segments@n\endcsname} {
        \ifnumcomp{\csname tt@carried@segment@\i @visited\endcsname}{=}{0}{
            \expandafter\xdef\csname tt@carried@segment@\i @visited\endcsname{1}
            \path[spath/save=tt@carried@tmpa] [tt/@carried dfs={\i}{begin}];
            \path[spath/save=tt@carried@tmpb] [spath/use={tt@carried@tmpa,reverse},spath/use={tt@carried@segment@\i},tt/@carried dfs={\i}{end}];
            \tikzset{
                spath/spot weld={tt@carried@tmpb},
                tt/add branch={\tt@carried@name}{[spath/use=tt@carried@tmpb]}
            }
        }{}
    }
    \ifnumcomp{\tt@carried@debug}{=}{1}{
        \ifnumcomp{\csname TT@\tt@carried@name @branches@n\endcsname}{>}{0}{
            \foreach \b in {1,...,\csname TT@\tt@carried@name @branches@n\endcsname} {
                \pgfmathparse{\b/(\csname TT@\tt@carried@name @branches@n\endcsname)}
                \definecolor{tt@mycolor}{hsb}{\pgfmathresult,1,1}
                \draw[tt@mycolor] [spath/use=\ttbranch{\tt@carried@name}{\b}];
            }
        }{}
        \foreach \s in {1,...,\csname TT@#1@switches@n\endcsname} {
            \foreach \dir in {l,r} {
                \ifnumcomp{\csname tt@carried@carrying@switch@\s @adj@\dir @n\endcsname}{>}{0}{
                    \foreach \i in {1,...,\csname tt@carried@carrying@switch@\s @adj@\dir @n\endcsname} {
                        \node[red,scale=.3] at (tt@carried@carrying@switch@\s @adj@\dir @\i @point) {\tikzcontour{\i}};
                    }
                }{}
            }
        }
        \ifnumcomp{\csname TT@\tt@carried@name @switches@n\endcsname}{>}{0}{
            \foreach \z in {1,...,\csname TT@\tt@carried@name @switches@n\endcsname} {
                \fill[red] (\ttswitch{\tt@carried@name}{\z}) circle (1pt);
            }
        }{}
    }{}
},
% @carried dfs={segment}{end}
@carried dfs/.code 2 args={}{
    % \typeout{dfs #1 #2}
    \edef\ss{\csname tt@carried@segment@#1@#2@switch\endcsname}
    % \typeout{switch \ss}
    \ifnumcomp{\ss}{>}{0}{
        \edef\idx{\csname tt@carried@segment@#1@#2@idx\endcsname}
        \edef\dir{\csname tt@carried@segment@#1@#2@dir\endcsname}
        % \typeout{\csname tt@carried@carrying@switch@\ss @adj@\dir @\idx @afterpath\endcsname}
        \tikzset{/@expand style={\csname tt@carried@carrying@switch@\ss @adj@\dir @\idx @afterpath\endcsname}}
        \edef\mate{\csname tt@carried@carrying@switch@\ss @adj@\dir @\idx @mate\endcsname}
        % \typeout{idx \idx\space dir \dir\space mate \mate}
        \ifnumcomp{\mate}{>}{0}{
            \edef\dir{\ifnumcomp{\pdfstrcmp{\dir}{l}}{=}{0}{r}{l}}
            \edef\nextsegment{\csname tt@carried@carrying@switch@\ss @adj@\dir @\mate @idx\endcsname}
            \ifnumcomp{\csname tt@carried@segment@\nextsegment @visited\endcsname}{=}{0}{
                \expandafter\xdef\csname tt@carried@segment@\nextsegment @visited\endcsname{1}
                \ifnumcomp{\pdfstrcmp{\csname tt@carried@carrying@switch@\ss @adj@\dir @\mate @end\endcsname}{begin}}{=}{0}{
                    \tikzset{
                        spath/use={tt@carried@segment@\nextsegment},
                        tt/@carried dfs={\nextsegment}{end}
                    }
                }{
                    \tikzset{
                        spath/use={tt@carried@segment@\nextsegment,reverse},
                        tt/@carried dfs={\nextsegment}{begin}
                    }
                }
            }{}
        }{}
    }{}
},
point along branch/.code n args={3}{
    \pgfinterruptboundingbox
    \xdef\tt@parsepointalongbranch@dx{0pt}
    \xdef\tt@parsepointalongbranch@end{begin}
    \xdef\tt@parsepointalongbranch@name{tt@p}
    \tikzset{tt/@parse point along branch/.cd,/@expand style={#3}}
    % \typeout{dx=\tt@parsepointalongbranch@dx}
    \ifthenelse{\equal{\tt@parsepointalongbranch@end}{begin}}{
        \scoped[spath/transform to={\ttbranch{#1}{#2}}{0}]\path[spath/save global=tt@path] ({\tt@parsepointalongbranch@dx},-10) -- +(0,20);
    }{
        \scoped[spath/transform to={\ttbranch{#1}{#2}}{0.999}]\path[spath/save global=tt@path] ({-(\tt@parsepointalongbranch@dx)},-10) -- +(0,20); 
    }
    \path[name path=tt@path] [spath/use=tt@path];
    \path[name path=tt@path2] [spath/use=\ttbranch{#1}{#2}];
    \tikzset{name intersections={of=tt@path and tt@path2,name=tt@,sort by=tt@path2,total=\tt@total}}
    \ifthenelse{\tt@total=0}{
        \PackageError{tt}{Branch #2 is too short}
    }{
        \ifthenelse{\equal{\tt@parsepointalongbranch@end}{begin}}{
            \coordinate (\tt@parsepointalongbranch@name) at (tt@-1);
        }{
            \coordinate (\tt@parsepointalongbranch@name) at (tt@-\tt@total);
        }
        % \fill[red] (\tt@parsepointalongbranch@name) circle (.5pt);
    }
    \endpgfinterruptboundingbox
},
@find closest switch/.code n args={3}{
    \edef\tt@r{#3}
    \xdef\tt@i{0}
    \ifnumcomp{\csname TT@#1@switches@n\endcsname}{>}{0}{
        \foreach \i in {1,...,\csname TT@#1@switches@n\endcsname}{
            \tikzmath{
                coordinate \a;
                \a=(\ttswitch{#1}{\i})-(#2);
                \r=veclen(\a);
                if \r<\tt@r then {
                    {\xdef\tt@r{\r}\xdef\tt@i{\i}};
                };
            }
        }
    }{}
    \xdef\tt@result{\tt@i}
},
}

\NewDocumentCommand{\tt@createpathretrievalcommands}{mmmm}{
    \tikzset{
        tt/.cd,
        #1/.code 2 args={
            \foreach #3 in {##2} {
                \tikzset{spath/use=tt@##1@#4}
            }
        },
        #1 all/.code={
            \foreach #3 in {1,...,\csname TT@##1@#2\endcsname} {
                \tikzset{spath/use=tt@##1@#4}
            }
        },
        #1 all but/.code 2 args={
            \foreach #3 in {1,...,\csname TT@##1@#2\endcsname} {
                \xdef\tt@createpathretrievalcommands@ok{1}
                \foreach \tt@createpathretrievalcommands@i in {##2} {
                    \ifthenelse{#3=\tt@createpathretrievalcommands@i}{
                        \xdef\tt@createpathretrievalcommands@ok{0}
                    }{}
                }
                \ifthenelse{\tt@createpathretrievalcommands@ok=1}{
                    \tikzset{spath/use=tt@##1@#4}
                }{}
            }
        }
    }
}

\tt@createpathretrievalcommands{use branch}{branches@n}{\b}{branch@\b}

\tt@createpathretrievalcommands{use switch upper contour}{switches@n}{\s}{switch@\s @upper contour}
\tt@createpathretrievalcommands{use switch lower contour}{switches@n}{\s}{switch@\s @lower contour}
\tt@createpathretrievalcommands{use switch contour}{switches@n}{\s}{switch@\s @contour}
\tt@createpathretrievalcommands{use switch background}{switches@n}{\s}{switch@\s @background}

\tt@createpathretrievalcommands{use branch left contour}{branches@n}{\b}{branch@\b @left contour}
\tt@createpathretrievalcommands{use branch right contour}{branches@n}{\b}{branch@\b @right contour}
\tt@createpathretrievalcommands{use branch contour}{branches@n}{\b}{branch@\b @contour}
\tt@createpathretrievalcommands{use branch background}{branches@n}{\b}{branch@\b @background}

\NewExpandableDocumentCommand{\ttswitch}{mm}{tt@#1@switch@#2}
\NewExpandableDocumentCommand{\ttbranch}{mm}{tt@#1@branch@#2}

\NewDocumentCommand{\tt@ensurefinalised}{m}{
    \ifthenelse{\boolean{TT@#1@isfinalised}}{}{\PackageWarning{tt}{Train track #1 is not finalised yet}}
}
\NewDocumentCommand{\tt@ensurenotfinalised}{m}{
    \ifthenelse{\boolean{TT@#1@isfinalised}}{\PackageWarning{tt}{Train track #1 is already finalised}}{}
}

\tikzset{
tt/@parse point along branch/.is family,
tt/@parse point along branch/.cd,
.unknown/.code={\xdef\tt@parsepointalongbranch@dx{\pgfkeyscurrentname}},
begin/.code={\xdef\tt@parsepointalongbranch@end{begin}},
end/.code={\xdef\tt@parsepointalongbranch@end{end}},
away from/.code={\TODO},
name/.code={\xdef\tt@parsepointalongbranch@name{#1}},
}

\tikzset{
tt/@parse carried/.is family,
tt/@parse carried/.cd,
defaults/.code={
    \gdef\tt@carried@name{\PackageWarning{tt}{Please set the name for the carried train track}}
    \xdef\tt@carried@debug{0}
    \foreach \z in {1,...,\csname TT@\tt@carried@carrying@name @switches@n\endcsname} {
        \expandafter\xdef\csname tt@carried@carrying@switch@\z @matches\endcsname{}
    }
    \foreach \i in {1,...,\csname TT@\tt@carried@carrying@name @branches@n\endcsname} {
        \expandafter\xdef\csname tt@carried@carrying@branch@\i @n\endcsname{0}
    }
},
name/.code={
    \xdef\tt@carried@name{#1}
    \tikzset{tt/new=#1}
},
switch/.code n args={4}{
    \tikzset{tt/add switch={\tt@carried@name}{[yshift=#2]\ttswitch{\tt@carried@carrying@name}{#1}}}
    \edef\s{\csname TT@\tt@carried@name @switches@n\endcsname}
    \expandafter\xdef\csname tt@carried@switch@\s @parentswitch\endcsname{#1}
    \expandafter\xdef\csname tt@carried@switch@\s @adj@l\endcsname{#3}
    \expandafter\xdef\csname tt@carried@switch@\s @adj@r\endcsname{#4}
},
debug/.code={
    \xdef\tt@carried@debug{1}
},
matches/.code 2 args={
    \expandafter\xdef\csname tt@carried@carrying@switch@#1@matches\endcsname{#2}
},
.unknown/.code={
    \expandafter\xdef\csname tt@carried@carrying@branch@\pgfkeyscurrentname @n\endcsname{#1}
},
}


\NewDocumentCommand{\tt@processbunchgenericpre}{mmmm}{
    \xdef\tt@processbunch@found{0}
    \tt@ifinproplist{TT@#1@switch@#2@bunches}{#4}{
        \xdef\tt@processbunch@n{0}
        \xdef\tt@processbunch@spread{\csname TT@#1@switch@#2@spread@#3\endcsname}
        \xdef\tt@processbunch@sep{\csname TT@#1@switch@#2@sep@#3\endcsname}
        \xdef\tt@processbunch@yshift{0}
        \xdef\tt@processbunch@found{1}
        % \typeout{Processing bunch "#4" of switch #2}
        \tikzset{tt/@parse bunch/.cd,/@expand style=\tt@result}
    }{}
}
\NewDocumentCommand{\tt@processbunchgenericpost}{mmm}{
    \edef\tt@sw{#2}
    \foreach \j in {1,...,\tt@processbunch@n} {
        \edef\n{\the\numexpr\csname TT@#1@branches@n\endcsname+1}
        \expandafter\xdef\csname TT@#1@branches@n\endcsname{\n}
        % \ifcsundef{TT@#1@branch@\j @weight}{
        %     \expandafter\xdef\csname TT@#1@branch@\n @weight\endcsname{0}
        % }{}
        \path[spath/save global=\ttbranch{#1}{\n}] (\ttswitch{#1}{\tt@sw}) to[out={90-(#3*90)},in={90+(#3*90)}] +({#3*(\tt@processbunch@spread)},{\tt@processbunch@firsty+(\tt@processbunch@yshift)-(\j-1)*(\tt@processbunch@sep)});
        \expandafter\xdef\csname TT@#1@branch@\n @begin\endcsname{\tt@sw}
        \expandafter\xdef\csname TT@#1@branch@\n @end\endcsname{0}
        \expandafter\xdef\csname TT@#1@branch@\n @frombunch\endcsname{1}
    }
}
\tikzset{
tt/@parse bunch/.is family,
tt/@parse bunch/.cd,
.unknown/.code={\pgfmathparse{\pgfkeyscurrentname}\xdef\tt@processbunch@n{\pgfmathresult}},
spread/.code={\xdef\tt@processbunch@spread{#1}},
sep/.code={\xdef\tt@processbunch@sep{#1}},
yshift/.code={\xdef\tt@processbunch@yshift{#1}},
}
\NewDocumentCommand{\tt@processbunchleft}{mm}{
    \tt@processbunchgenericpre{#1}{#2}{l}{left}
    \ifthenelse{\tt@processbunch@found=1}{
        \tt@addtosequence{TT@#1@bunches@left}{#2/\csname TT@#1@branches@n\endcsname/\tt@processbunch@n/\tt@processbunch@spread/\tt@processbunch@sep/\tt@processbunch@yshift}
        \tikzmath{\h=.5*(\tt@processbunch@n-1)*(\tt@processbunch@sep);}
        \xdef\tt@processbunch@firsty{\h}
        \tt@processbunchgenericpost{#1}{#2}{-1}
    }{}
}
\NewDocumentCommand{\tt@processbunchright}{mm}{
    \tt@processbunchgenericpre{#1}{#2}{r}{right}
    \ifthenelse{\tt@processbunch@found=1}{
        \tt@addtosequence{TT@#1@bunches@right}{#2/\csname TT@#1@branches@n\endcsname/\tt@processbunch@n/\tt@processbunch@spread/\tt@processbunch@sep/\tt@processbunch@yshift}
        \tikzmath{\h=.5*(\tt@processbunch@n-1)*(\tt@processbunch@sep);}
        \xdef\tt@processbunch@firsty{\h}
        \tt@processbunchgenericpost{#1}{#2}{1}
    }{}
}
\NewDocumentCommand{\tt@processbunchabove}{mmmmm}{
    \tt@processbunchgenericpre{#1}{#2}{#3}{above #4}
    \ifthenelse{\tt@processbunch@found=1}{
        \ifthenelse{\equal{#3}{l}}{
            \def\tt@dirmult{-1}
        }{
            \def\tt@dirmult{1}
        }
        \tt@addtosequence{TT@#1@bunches@above}{#4/#5/\tt@dirmult/\csname TT@#1@branches@n\endcsname/\tt@processbunch@n/\tt@processbunch@spread/\tt@processbunch@sep/\tt@processbunch@yshift}
        \tikzset{tt/point along branch={#1}{#4}{\tt@processbunch@spread,#5,name=tt@p}}
        \tikzmath{coordinate \p;\p=(tt@p)-(\ttswitch{#1}{#2});\h=\py+\tt@processbunch@n*(\tt@processbunch@sep);}
        \xdef\tt@processbunch@firsty{\h}
        \tt@processbunchgenericpost{#1}{#2}{\tt@dirmult}
    }{}
}
\NewDocumentCommand{\tt@processbunchbelow}{mmmmm}{
    \tt@processbunchgenericpre{#1}{#2}{#3}{below #4}
    \ifthenelse{\tt@processbunch@found=1}{
        \ifthenelse{\equal{#3}{l}}{
            \def\tt@dirmult{-1}
        }{
            \def\tt@dirmult{1}
        }
        \tt@addtosequence{TT@#1@bunches@below}{#4/#5/\tt@dirmult/\csname TT@#1@branches@n\endcsname/\tt@processbunch@n/\tt@processbunch@spread/\tt@processbunch@sep/\tt@processbunch@yshift}
        \tikzset{tt/point along branch={#1}{#4}{\tt@processbunch@spread,#5,name=tt@p}}
        \tikzmath{coordinate \p;\p=(tt@p)-(\ttswitch{#1}{#2});\h=\py-(\tt@processbunch@sep);}
        \xdef\tt@processbunch@firsty{\h}
        \tt@processbunchgenericpost{#1}{#2}{\tt@dirmult}
    }{}
}
\NewDocumentCommand{\tt@processbunchbetween}{mmmmmmm}{
    \tt@processbunchgenericpre{#1}{#2}{#3}{between #4 and #6}
    \ifthenelse{\tt@processbunch@found=1}{
        \ifthenelse{\equal{#3}{l}}{
            \def\tt@dirmult{-1}
        }{
            \def\tt@dirmult{1}
        }
        \tt@addtosequence{TT@#1@bunches@between}{#4/#5/#6/#7/\tt@dirmult/\csname TT@#1@branches@n\endcsname/\tt@processbunch@n/\tt@processbunch@spread/\tt@processbunch@yshift}
        \tikzset{tt/point along branch={#1}{#4}{\tt@processbunch@spread,#5,name=tt@pt}}
        \tikzset{tt/point along branch={#1}{#6}{\tt@processbunch@spread,#7,name=tt@pb}}
        \tikzmath{
            coordinate \p;
            \p=(tt@pt)-(tt@pb);
            \s=\py/(\tt@processbunch@n+1);
            \p=(tt@pt)-(\ttswitch{#1}{#2});
            \h=\py-\s;
        }
        \xdef\tt@processbunch@firsty{\h}
        \xdef\tt@processbunch@sep{\s pt}
        \tt@processbunchgenericpost{#1}{#2}{\tt@dirmult}
    }
}

% \tt@thick@processbunchgeneric{traint track}{1/-1 for direction}
\NewDocumentCommand{\tt@thick@processbunchgeneric}{mm}{
    \pgfmathparse{\tt@firsty+(\tt@yshift)}
    \edef\tt@y{\pgfmathresult}
    \tikzmath{
        coordinate \a;
        \k=int(\tt@beg+1);
        \a=(tt@branch@\k @newbegin);
        \tt@x=\ax+\tt@spread*(#2);
    }
    \foreach \i[evaluate=\i as \j using int(\tt@beg+\i)] in {1,...,\tt@n} {
        \pgfmathparse{\tt@y-(\csname TT@#1@branch@\j @thickness\endcsname)/2}
        \xdef\tt@y{\pgfmathresult}
        \path[spath/save global=\ttbranch{#1}{\j}] (tt@branch@\j @newbegin) to[out={90-(#2*90)},in={90+(#2*90)}] (\tt@x pt,\tt@y pt);
        \pgfmathparse{\tt@y-(\csname TT@#1@branch@\j @thickness\endcsname)/2-\tt@sep}
        \xdef\tt@y{\pgfmathresult}
    }
}
\NewDocumentCommand{\tt@thick@processbunchleft}{mm}{
    \foreach \sw/\tt@beg/\tt@n/\tt@spread/\tt@sep/\tt@yshift in #2 {
        \tt@gettotalthickness{#1}{\tt@beg}{\tt@n}
        \edef\tt@totalthickness{\tt@result}
        % \typeout{Total thickness is \tt@totalthickness}
        \tikzmath{
            coordinate \a;
            \a=(\ttswitch{#1}{\sw});
        }
        \pgfmathsetmacro{\tt@firsty}{\ay+(\tt@totalthickness+\tt@sep*(\tt@n-1))/2}
        \tt@thick@processbunchgeneric{#1}{-1}
    }
}
\NewDocumentCommand{\tt@thick@processbunchright}{mm}{
    \foreach \sw/\tt@beg/\tt@n/\tt@spread/\tt@sep/\tt@yshift in #2 {
        \tt@gettotalthickness{#1}{\tt@beg}{\tt@n}
        \edef\tt@totalthickness{\tt@result}
        % \typeout{Total thickness is \tt@totalthickness}
        \tikzmath{
            coordinate \a;
            \a=(\ttswitch{#1}{\sw});
        }
        \pgfmathsetmacro{\tt@firsty}{\ay+(\tt@totalthickness+\tt@sep*(\tt@n-1))/2}
        \tt@thick@processbunchgeneric{#1}{1}
    }
}
\NewDocumentCommand{\tt@thick@processbunchabove}{mm}{
    \foreach \br/\end/\dirmult/\tt@beg/\tt@n/\tt@spread/\tt@sep/\tt@yshift in #2 {
        \tt@gettotalthickness{#1}{\tt@beg}{\tt@n}
        \edef\tt@totalthickness{\tt@result}
        \tikzset{tt/point along branch={#1}{\br}{\tt@spread,\end,name=tt@p}}
        \tikzmath{
            coordinate \a;
            \a=(tt@p);
        }
        \pgfmathsetmacro{\tt@firsty}{\ay+\tt@totalthickness+\tt@sep*\tt@n+\csname TT@#1@branch@\br @thickness\endcsname/2}
        \tt@thick@processbunchgeneric{#1}{\dirmult}
    }
}
\NewDocumentCommand{\tt@thick@processbunchbelow}{mm}{
    \foreach \br/\end/\dirmult/\tt@beg/\tt@n/\tt@spread/\tt@sep/\tt@yshift in #2 {
        \tikzset{tt/point along branch={#1}{\br}{\tt@spread,\end,name=tt@p}}
        \tikzmath{
            coordinate \a;
            \a=(tt@p);
        }
        \pgfmathsetmacro{\tt@firsty}{\ay-\tt@sep-\csname TT@#1@branch@\br @thickness\endcsname/2}
        \tt@thick@processbunchgeneric{#1}{\dirmult}
    }
}
\NewDocumentCommand{\tt@thick@processbunchbetween}{mm}{
    \foreach \br/\end/\brr/\endd/\dirmult/\tt@beg/\tt@n/\tt@spread/\tt@yshift in #2 {
        \tikzset{tt/point along branch={#1}{\br}{\tt@spread,\end,name=tt@pt}}
        \tikzset{tt/point along branch={#1}{\brr}{\tt@spread,\endd,name=tt@pb}}
        \tt@gettotalthickness{#1}{\tt@beg}{\tt@n}
        \edef\tt@totalthickness{\tt@result}
        \tikzmath{
            coordinate \p;
            \p=(tt@pt)-(tt@pb);
            \tt@sep=(\py-\tt@totalthickness)/(\tt@n+1);
            \p=(tt@pt);
        }
        \pgfmathsetmacro{\tt@firsty}{\py-\tt@sep-\csname TT@#1@branch@\br @thickness\endcsname/2}
        \tt@thick@processbunchgeneric{#1}{\dirmult}
    }
}

% \tt@gettotalthickness{train track}{begin-1}{count}
\NewDocumentCommand{\tt@gettotalthickness}{mmm}{
    \xdef\tt@result{0}
    \foreach \i[evaluate=\i as \j using int(#2+\i)] in {1,...,#3} {
        \pgfmathparse{\tt@result+\csname TT@#1@branch@\j @thickness\endcsname}
        \xdef\tt@result{\pgfmathresult}
    }
}

\NewDocumentCommand{\tt@adjustendpointsofbranch}{mmm}{
    \tikzset{spath/replace lines=#1}
    \xdef\tt@adjustendpoints@n{1}
    \path[decorate,decoration={show path construction,
        curveto code={
            \coordinate (tt@adjustendpoints@\tt@adjustendpoints@n) at (\tikzinputsegmentfirst);
            \coordinate (tt@adjustendpoints@controla@\tt@adjustendpoints@n) at (\tikzinputsegmentsupporta);
            \coordinate (tt@adjustendpoints@controlb@\tt@adjustendpoints@n) at (\tikzinputsegmentsupportb);
            \xdef\tt@adjustendpoints@n{\the\numexpr\tt@adjustendpoints@n+1}
            \coordinate (tt@adjustendpoints@\tt@adjustendpoints@n) at (\tikzinputsegmentlast);
        }
    }] [spath/use=#1];
    \coordinate (tt@adjustendpoints@controla@1) at ($(tt@adjustendpoints@controla@1)-(tt@adjustendpoints@1)+(#2)$);
    \pgfmathparse{int(\tt@adjustendpoints@n-1)}
    \coordinate (tt@adjustendpoints@controlb@\pgfmathresult) at ($(tt@adjustendpoints@controlb@\pgfmathresult)-(tt@adjustendpoints@\tt@adjustendpoints@n)+(#3)$);
    \coordinate (tt@adjustendpoints@1) at (#2);
    \coordinate (tt@adjustendpoints@\tt@adjustendpoints@n) at (#3);
    \path[spath/save global=#1] (tt@adjustendpoints@1) \foreach \i[evaluate=\i as \i using {int(\i)},evaluate=\i as \j using {int(\i-1)}] in {2,...,\tt@adjustendpoints@n} { .. controls (tt@adjustendpoints@controla@\j) and (tt@adjustendpoints@controlb@\j) .. (tt@adjustendpoints@\i) };
}

\tikzset{
    spath/offset/.code n args={3}{
        \tt@offsetpath{#1}{#2}{#3}
    }
}

\ExplSyntaxOn

\NewDocumentCommand{\tt@offsetpath}{mmm}{
    \pgfinterruptboundingbox
    \path[save~path=\tt@offsetpath@tmppath] [spath/use=#1];
    \pgfoffsetpath{\tt@offsetpath@tmppath}{#2}
    \spath_get_current_path:N \tt@offsetpath@tmppath
    \pgfusepath{discard}
    \tl_gclear_new:c {\__tikzspath_path_name:n {#3}}
    \tl_gset:cV {\__tikzspath_path_name:n {#3}} \tt@offsetpath@tmppath
    \endpgfinterruptboundingbox
}

\NewDocumentCommand{\tt@newproplist}{m}{
    \prop_gclear_new:c { #1 }
}
\NewDocumentCommand{\tt@addtoproplist}{mmm}{
    \tl_set:Ne \l_tmpa_tl { #2 }
    % \typeout{Adding~"\l_tmpa_tl"~to~#1}
    \prop_gput:cen { #1 } { \l_tmpa_tl } { #3 }
}
\NewDocumentCommand{\tt@ifinproplist}{mmmm}{
    \tl_set:Ne \l_tmpb_tl { #2 }
    \prop_gpop:ceNTF { #1 } { \l_tmpb_tl } \l_tmpa_tl { \edef\tt@result{\tl_use:N \l_tmpa_tl} #3 } { #4 }
}
\NewDocumentCommand{\tt@proplistlength}{m}{
    \prop_count:c { #1 }
}

\cs_generate_variant:Nn \tl_set:Nn {Ne}
\cs_generate_variant:Nn \prop_gput:Nnn {cen}
\cs_generate_variant:Nn \prop_gpop:NnNTF {ceNTF}

\NewDocumentCommand{\tt@newsequence}{m}{
    \seq_gclear_new:c { #1 }
}
\NewDocumentCommand{\tt@sequencelength}{m}{
    \seq_count:c { #1 }
}
\NewDocumentCommand{\tt@addtosequence}{mm}{
    \seq_gput_left:cx { #1 } { #2 }
}
\NewExpandableDocumentCommand{\tt@getfromsequence}{mm}{
    \seq_item:cn { #1 } { #2 }
}
\NewDocumentCommand{\tt@showsequence}{m}{
    \seq_show:c { #1 }
}

\NewDocumentCommand{\tt@sortadjacencylist}{mm}{
    % \seq_show:c { #1 }
    \seq_sort:cn { #1 } {
        \seq_set_split:Nnn \l_tmpa_seq { , } { ##1 }
        \seq_get_left:NN \l_tmpa_seq \l_tmpa_tl
        \seq_set_split:Nnn \l_tmpb_seq { , } { ##2 }
        \seq_get_left:NN \l_tmpb_seq \l_tmpb_tl
        \dim_compare:nNnTF { \l_tmpa_tl } < { \l_tmpb_tl } { \sort_return_same: } { \sort_return_swapped: }
    }
    \seq_set_eq:Nc \l_tmpa_seq { #1 }
    \seq_gclear:c { #1 }
    \seq_gclear_new:c { #2 }
    \seq_map_inline:Nn \l_tmpa_seq {
        \seq_set_split:Nnn \l_tmpb_seq { , } { ##1 }
        \seq_gput_left:cx { #1 } { \seq_item:Nn \l_tmpb_seq 2 }
        \seq_gput_left:cx { #2 } { \seq_item:Nn \l_tmpb_seq 3 }
    }
}

\NewDocumentCommand{\tt@warnforinvalidbunches}{mm}{
    \prop_map_inline:cn { #2 } {
        \PackageWarning{tt}{Bunch~##1~of~switch~#1~is~invalid}
    }
}

\ExplSyntaxOff

\makeatother
